Delta Function Scattering with Feynman Diagrams in 1d Quantum Mechanics

In this paper we will demonstrate the use of Feynman Diagrams for one dimensional scattering in quantum mechanics. We will evaluate the S-Matrix explicitly for the Dirac delta and finite wall potentials by summing the full series of Feynman diagrams, illustrating the spirit of perturbation theory. This technique may be useful in introductory quantum mechanics courses, and provides the student with intuition about conservation laws in the context of scattering problems by connecting Feynman diagrams, free propagation, and conservation of the corresponding observable. It also provides a toy model for calculating S-matrix elements in quantum field theory.

==> sn-bibliography.tex <==
\bibitem{bib1} D. Griffiths, Introduction to Quantum Mechanics, Cambridge University Press, 2005.

\bibitem{bib2} R. Shankar, Principles of Quantum Mechanics, Plenum Press, New York, 1994.

\bibitem{bib3} K. Gottfried, Quantum Mechanics: Fundamentals, Springer, 1966.

\bibitem{bib4} M. Peskin, D. Schroeder, An Introduction to Quantum Field Theory, CRC Press LLC, 2019.
